Stochastic Variance-Reduced Heavy Ball Power Iteration

We present a stochastic variance-reduced heavy ball power iteration algorithm for solving PCA and provide a convergence analysis for it. The algorithm is an extension of heavy ball power iteration, incorporating a step size so that progress can be controlled depending on the magnitude of the variance of stochastic gradients. The algorithm works with any size of the mini-batch, and if the step size is appropriately chosen, it attains global linear convergence to the first eigenvector of the covariance matrix in expectation. The global linear convergence result in expectation is analogous to those of stochastic variance-reduced gradient methods for convex optimization but due to non-convexity of PCA, it has never been shown for previous stochastic variants of power iteration since it requires very different techniques. We provide the first such analysis and stress that our framework can be used to establish convergence of the previous stochastic algorithms for any initial vector and in expectation. Experimental results show that the algorithm attains acceleration in a large batch regime, outperforming benchmark algorithms especially when the eigen-gap is small.

==> technical-lemma.tex <==
\begin{lemma} \label{lemma:trace}
Let $w$ be a vector in $\mathbb{R}^d$, and $P$, $M$ be $d \times d$ symmetric matrices. Then, we have
\begin{align*}
w^TPMPw \leq \| M \| \| Pw \|^2.
\end{align*}
\end{lemma}
\begin{proof}
By the cyclic property of the trace, we have
\begin{align*}
w^TPMPw = \text{Tr}[w^TPMPw] = \text{Tr}[MPww^TP].
\end{align*}
From that $Pww^TP$ is positive semi-definite, we have
\begin{align*}
\text{Tr}[MPww^TP] \leq \| M \| \text{Tr}[Pww^TP].
\end{align*}
Again, by the cyclic property of the trace, we finally have
\begin{align*}
w^TPMPw \leq \| M \| \text{Tr}[Pww^TP] = \| M \| \text{Tr}[w^TPPw] = \| M \| \| Pw \|^2.
\end{align*}
\end{proof}

\begin{lemma} \label{lemma:linear-algebra}
Let $w$ be a vector in $\mathbb{R}^d$ with $\|w\|=1$ and $C$ be a $d \times d$ symmetric matrix. Then, for $P=I-ww^T$, we have
\begin{align*} 
\| PC - CP \|_2^2 = w^TC^2w - (w^TCw)^2.
\end{align*}
\end{lemma}
\begin{proof}
By definition of $P$, we have
\begin{align*}
PC - CP = (I - ww^T)C - C(I-ww^T) = Cww^T - ww^TC,
\end{align*}
resulting in
\begin{align*}
(PC - CP)^T(PC - CP) &= (Cww^T - ww^TC)^T(Cww^T - ww^TC) \\
&= ww^TC^2ww^T - ww^TCww^TC - Cww^TCww^T + Cww^Tww^TC \\
&= (w^TC^2w)ww^T - (w^TCw)ww^TC - (w^TCw)Cww^T + Cww^TC.
\end{align*}
For any vector $u$ in $\mathbb{R}^d$, we have
\begin{align*}
(PC - CP)^T(PC - CP)u &= (w^TC^2w)ww^Tu - (w^TCw)ww^TCu - (w^TCw)Cww^Tu + Cww^TCu \\
&= \big[ (w^TC^2w)(w^Tu) - (w^TCw)(w^TCu) \big]w + \big[w^TCu - (w^TCw)(w^Tu) \big] Cw,
\end{align*}
meaning that $(PC - CP)^T(PC - CP)u$ lies in the span of $w$ and $Cw$. Therefore, any eigenvector which does not belong to the span of $w$ and $Cw$ must have an eigenvalue of zero. 

For
\begin{align}
u = c_1w + c_2 Cw, \label{eq:linear-algebra-u}
\end{align}
we have
\begin{align*}
(PC - CP)^T(PC - CP)u &= c_1[ (w^TC^2w) - (w^TCw)^2 ]w + c_2[w^TC^2w - (w^TCw)^2] Cw \\
&= [ (w^TC^2w) - (w^TCw)^2 ] (c_1w + c_2Cw) \\
&= [ (w^TC^2w) - (w^TCw)^2 ] u.
\end{align*}
Therefore, any vector $u$ in the form of \eqref{eq:linear-algebra-u} is an eigenvector of $(PC - CP)^T(PC - CP)$ with an eigenvalue of 
\begin{align*}
w^TC^2w - (w^TCw)^2 = \| (I - ww^T) Cw \|^2 \geq 0,
\end{align*}
resulting in
\begin{align*}
\| PC - CP \|^2 = w^TC^2w - (w^TCw)^2.
\end{align*}
\end{proof}

\begin{lemma} \label{lemma:quadratic-form}
Let $C$ be a $d \times d$ symmetric, positive semidefinite matrix and $(\lambda_1,u_1)$ be the largest eigenpair of $C$. Then, for any unit vector $w$ in $\mathbb{R}^d$, we have
\begin{align*} 
w^TC^2w - (w^TCw)^2 \leq 2 \lambda_1^2(1-(u_1^Tw)^2).
\end{align*}
\end{lemma}

\begin{proof}
From
\begin{align*}
w = (u_1^Tw) u_1 + (I - u_1u_1^T) w,
\end{align*}
we have
\begin{align*}
w^TCw &= \lambda_1(u_1^T w)^2 + w^T(I-u_1u_1^T)C(I-u_1u_1^T)w
\end{align*}
and
\begin{align*}
w^TC^2w &= \lambda_1^2(u_1^T w)^2 + w^T(I-u_1u_1^T)C^2(I-u_1u_1^T)w,
\end{align*}
leading to
\begin{align*}
\lambda_1(u_1^Tw)^2 \leq w^TCw \leq \lambda_1, \quad \lambda_1^2(u_1^Tw)^2 \leq w^TC^2w \leq \lambda_1^2.
\end{align*}
Therefore,
\begin{align*}
w^TC^2w - (w^TCw)^2 \leq \lambda_1^2(1-(u_1^Tw)^4) = 2 \lambda_1^2(1+(u_1^Tw)^2)(1-(u_1^Tw)^2) \leq 2 \lambda_1^2( 1-(u_1^Tw)^2)
\end{align*}
where the last inequality follows from $(u_1^Tw)^2 \leq \|u_1\|^2 \|w\|^2 = 1$.
\end{proof}

\begin{lemma} \label{lemma:coefficient-inequality}
Let $w_t$ be a sequence of real numbers such that
\begin{align*}
w_t = (\alpha-\beta) w_{t-1} - \beta (\alpha-\beta) w_{t-2} + \beta^3 w_{t-3} + L_{t-1} + \beta L_{t-2}
\end{align*}
for $t \geq 3$ and $w_0 = L_0, w_1 = \alpha L_0, w_2 = (\alpha-\beta)^2L_0 + L_{1}$. Then, we have
\begin{align}
w_t = p_{t}(\alpha,\beta) L_0 + \sum_{r=1}^{t-1} p_{t-r-1}(\alpha,\beta) L_{r} \label{eq:coefficient-expression}
\end{align}
where $p_t(\alpha,\beta)$ is a recurrence polynomial defined as
\begin{align}
p_t(\alpha,\beta) &= (\alpha - \beta) p_{t-1}(\alpha,\beta) - \beta (\alpha - \beta) p_{t-2}(\alpha,\beta) + \beta^3 p_{t-3}(\alpha,\beta) \label{eq:coefficient-relation-p}
\end{align}
for $t \geq 3$ with
\begin{align}
p_0(\alpha,\beta) = 1, \quad p_1(\alpha,\beta) = \alpha, \quad p_2(\alpha,\beta) = (\alpha-\beta)^2.
\label{eq:coefficient-initial-condition}
\end{align}
Moreover, for $t \geq 0$, we have
\begin{itemize}
\item if $0 \leq 4 \beta < \alpha$, \begin{align}
p_t(\alpha,\beta) \geq 0. \label{eq:coefficient-positivity-general-alpha}
\end{align}
\item if $0 \leq \alpha = 4\beta$,
\begin{align}
p_t(4\beta,\beta) = (t+1)^2 \beta^t \geq 0. \label{eq:coefficient-positivity-special-alpha}
\end{align}
\item if $0 \leq \alpha < 4 \beta$, \begin{align}
p_t(\alpha,\beta) \leq p_t(4\beta,\beta). \label{eq:coefficient-inequality}
\end{align}
\end{itemize}
\end{lemma}

\begin{proof}
It is easy to check that $w_0$, $w_1$, and $w_2$ satisfy \eqref{eq:coefficient-expression}. Suppose that \eqref{eq:coefficient-expression} holds for $t-1,t-2,t-3$. Then, we have
\begin{align*}
w_t &= (\alpha-\beta) w_{t-1} - \beta (\alpha-\beta) w_{t-2} + \beta^3 w_{t-3} + L_{t-1} + \beta L_{t-2} \\
&= p_{t}(\alpha,\beta) L_0 + L_{t-1} + \alpha L_{t-2} + (\alpha-\beta)^2 L_{t-3} + \sum_{r=1}^{t-4} p_{t-r-1}(\alpha,\beta) L_r \\
&= p_{t}(\alpha,\beta) L_0  + \sum_{r=1}^{t-1} p_{t-r-1}(\alpha,\beta) L_{r}.
\end{align*}
Therefore, \eqref{eq:coefficient-expression} holds by induction.

Next, we prove \eqref{eq:coefficient-positivity-general-alpha}, \eqref{eq:coefficient-positivity-special-alpha} and \eqref{eq:coefficient-inequality}. The characteristic equation of \eqref{eq:coefficient-relation-p} is
\begin{align}
r^3 - (\alpha-\beta) r^2 + \beta (\alpha-\beta) r - \beta^3 = 0. \label{eq:characteristic-equation}
\end{align}
If $0 \leq 4\beta < \alpha$, the roots of \eqref{eq:characteristic-equation} are 
\begin{align*}
r = \beta, \frac{\alpha-2\beta}{2} + \frac{\sqrt{\alpha^2-4\alpha\beta}}{2}, \frac{\alpha-2\beta}{2} - \frac{\sqrt{\alpha^2-4\alpha\beta}}{2}.
\end{align*}
With initial conditions \eqref{eq:coefficient-initial-condition}, we obtain
\begin{align*}
p_t(\alpha,\beta) & = \frac{1}{\alpha - 4 \beta} \bigg[ \bigg( \frac{\alpha-2\beta}{2} + \frac{\sqrt{\alpha^2-4\alpha\beta}}{2} \bigg)^{t+1}  + \bigg( \frac{\alpha-2\beta}{2} - \frac{\sqrt{\alpha^2-4\alpha\beta}}{2} \bigg)^{t+1} - 2 \beta^{t+1} \bigg] \\
& = \frac{1}{\alpha - 4 \beta} \Bigg[ \bigg( \frac{\alpha-2\beta}{2} + \frac{\sqrt{\alpha^2-4\alpha\beta}}{2} \bigg)^{(t+1)/2}  - \bigg( \frac{\alpha-2\beta}{2} - \frac{\sqrt{\alpha^2-4\alpha\beta}}{2} \bigg)^{(t+1)/2} \Bigg]^2 \geq 0.
\end{align*}

If $0 \leq \alpha = 4\beta$, \eqref{eq:characteristic-equation} has a cube root of $r=\beta$.
From initial conditions \eqref{eq:coefficient-initial-condition}, we obtain
\begin{align}
p_t(4\beta,\beta) = (t+1)^2 \beta^t \geq 0.
\label{eq:polynomial-closed-form-special-alpha}
\end{align}

If $0 \leq \alpha < 4 \beta$, the roots of \eqref{eq:characteristic-equation} are 
\begin{align*}
r = \beta, \frac{\alpha-2\beta}{2} + \frac{\sqrt{4\alpha\beta-\alpha^2}}{2} i, \frac{\alpha-2\beta}{2} - \frac{\sqrt{4\alpha\beta-\alpha^2}}{2} i.
\end{align*}
Setting
\begin{align*}
\text{cos } \theta  = \frac{\alpha -2 \beta}{2\beta}, \quad \text{sin } \theta  = \frac{\sqrt{4\alpha\beta-\alpha^2}}{2\beta}, \quad \text{cos } \phi_p  = 1-\frac{\alpha}{2\beta}, \quad \text{sin } \phi_p  = -\frac{\sqrt{4\alpha\beta-\alpha^2}}{2\beta},
\end{align*}
it is easy to verify that
\begin{align}
p_t(\alpha,\beta) &= \bigg[ \frac{2\beta}{4\beta-\alpha} + \frac{2\beta}{4\beta-\alpha} \text{cos} (\phi_p + t \theta) \bigg] \beta^t.
\label{eq:polynomial-closed-form-general-alpha-trigonometric-p}
\end{align}
Let
\begin{align*}
P(t) = \frac{p_t(4\beta,\beta) - p_t(\alpha,\beta)}{\beta^t}.
\end{align*}
Then, from \eqref{eq:coefficient-relation-p} and \eqref{eq:coefficient-initial-condition}, we have
\begin{align}
P(0) = 0, \quad P(1) = \frac{4\beta - \alpha}{\beta}, \quad P(2)= \frac{(4\beta-\alpha)(2\beta+\alpha)}{\beta^2}, \quad P(3) = \frac{(\alpha^2 + 4\beta^2)(4\beta-\alpha)}{\beta^3}
\label{eq:polynomial-initial-condition-p-1}
\end{align}
resulting in
\begin{align}
P(2)-P(0) = \frac{(4\beta-\alpha)(2\beta+\alpha)}{\beta^2} \geq 0, \quad P(3)-P(1) = \frac{(\alpha^2 + 3\beta^2)(4\beta-\alpha)}{\beta^3} \geq 0. \label{eq:polynomial-initial-condition-p-2}
\end{align}
In order to show $P(t) \geq 0$ for $t \geq 0$, we prove $P(t+2)-P(t) \geq 0$ for $t \geq 0$. Using \eqref{eq:polynomial-closed-form-special-alpha}, \eqref{eq:polynomial-closed-form-general-alpha-trigonometric-p} and standard trigonometric equalities, it follows that
\begin{align*}
P(t+2)-2P(t)+P(t-2) = 8 + \frac{2\alpha}{\beta} \text{cos}(\phi_p + t\theta).
\end{align*}
In turn, we have
\begin{align}
P(t+2) - P(t) &= P(t) - P(t-2) + 8 + \frac{2\alpha}{\beta} \text{cos} (\phi+t\theta) \nonumber \\
&\geq P(t) - P(t-2) + 8 - \frac{2\alpha}{\beta} \nonumber \\
&= P(t) - P(t-2) + \frac{2(4\beta-\alpha)}{\beta} \nonumber \\
&\geq P(t) - P(t-2). \label{eq:coefficient-inequality-relation-p}
\end{align}
From \eqref{eq:polynomial-initial-condition-p-1}, \eqref{eq:polynomial-initial-condition-p-2}, and \eqref{eq:coefficient-inequality-relation-p}, we obtain $P(t) \geq 0$ for $t \geq 0$ implying
\begin{align*}
p_t(\alpha,\beta) \leq p_t(4\beta,\beta)
\end{align*}
for $t \geq 0$.
\end{proof}

\begin{lemma} \label{lemma:three-term-inequality-compact-form}
Let $w_t$ be a sequence of non-negative real numbers such that
\begin{align*}
w_t \leq \alpha w_{t-1} + \beta w_{t-2} + L_{t-1}
\end{align*}
for $t \geq 2$ with $w_0 = 0, L_0 \geq 0, \alpha \geq 0$ and $w_1 \leq L_0$. Then, we have
\begin{align}
w_t \leq q_{t}(\alpha,\beta) L_0 + \sum_{r=1}^{t-1} q_{t-r-1}(\alpha,\beta) L_{r} \label{eq:three-term-inequality-compact-form}
\end{align}
where $q_t(\alpha,\beta)$ is a recurrence polynomial defined as
\begin{align}
q_t(\alpha,\beta) &= \alpha q_{t-1}(\alpha,\beta) + \beta q_{t-2}(\alpha,\beta) \label{eq:coefficient-relation-q}
\end{align}
for $t \geq 2$ with
\begin{align}
q_0(\alpha,\beta) = 1, \quad q_1(\alpha,\beta) = \alpha.
\label{eq:coefficient-initial-condition-q}
\end{align}
\end{lemma}

\begin{proof}
From $w_0 = 0$ and $w_1 \leq L_0$, it is easy to check that \eqref{eq:three-term-inequality-compact-form} holds for $t = 0$ and $t=1$. Suppose that \eqref{eq:three-term-inequality-compact-form} holds for $t-1$ and $t-2$. Then, we have
\begin{align*}
w_t &\leq \alpha w_{t-1} + \beta w_{t-2} + L_{t-1} \\
&\leq \alpha ( q_{t-1}(\alpha,\beta) L_0 + \sum_{r=1}^{t-2} q_{t-r-2}(\alpha,\beta) L_{r} ) + \beta ( q_{t-2}(\alpha,\beta) L_0 + \sum_{r=1}^{t-3} q_{t-r-3}(\alpha,\beta) L_{r} ) + L_{t-1} \\
&= (\alpha q_{t-1}(\alpha,\beta) + \beta q_{t-2}(\alpha,\beta)) L_0 + L_{t-1} + \alpha L_{t-2} + \sum_{r=1}^{t-3} (\alpha q_{t-r-2}(\alpha,\beta) + \beta q_{t-r-3}(\alpha,\beta)) L_{r} \\
&= q_{t}(\alpha,\beta) L_0 + \sum_{r=1}^{t-1} q_{t-r-1}(\alpha,\beta) L_{r}.
\end{align*}
Therefore, by mathematical induction, \eqref{eq:three-term-inequality-compact-form} holds for every $t$.
\end{proof}


